Strategyproof Mechanism for Two Heterogeneous Facilities with Constant Approximation Ratio

In this paper, we study the two-facility location game on a line with optional preference where the acceptable set of facilities for each agent could be different and an agent's cost is his distance to the closest facility within his acceptable set. The objective is to minimize the total cost of all agents while achieving strategyproofness. We design a deterministic strategyproof mechanism for the problem with approximation ratio of 2.75, improving upon the earlier best ratio of n/2+1.

==> chap/chap_backup.tex <==


\par\vspace{1ex}\noindent\textbf{\Large Observation 2.2}\vspace{1ex}\par
We claim: to find the approximation ratio of Mechanism 2.1, we can assume $\forall i, p_i \ne \{\{F_1,F_2\}\}$.\par
Proof: Given any location profile \textbf{x}, we assume for preference profile \textbf{p}, $\exists i, p_i = \{F_1,F_2\}$. We let \textbf{p'} = $\{p_1 ,p_2, ..., p_{i-1}, p'_i, p_{i+1}, ..., p_n\}$, where $p'_i$ is $\{F_1\}$ if $dist(x_i,opt_{\textbf{p},1})<dist(x_i,opt_{\textbf{p},2})$, otherwise $p'_i$ is $\{F_2\}$. It is easy to find that $COST_{\textbf{p'}}(opt_{\textbf{p},1},opt_{\textbf{p},2})$ = $COST_{\textbf{p}}(opt_{\textbf{p},1},opt_{\textbf{p},2})$. Hence, we have $COST_{\textbf{p'}}(opt_{\textbf{p'},1},opt_{\textbf{p'},2}) \le COST_{\textbf{p'}}(opt_{\textbf{p},1},opt_{\textbf{p},2})$ = $COST_{\textbf{p}}(opt_{\textbf{p},1},opt_{\textbf{p},2})$.\par

Notice that for any $(y_1,y_2)$, $COST_{\textbf{p'}}(y_1,y_2) \ge COST_{\textbf{p}}(y_1,y_2)$. Given (\textbf{x},\textbf{p}) and (\textbf{x},\textbf{p'}) have the same location preference, the outputs of Mechanism 2.1 on them are the same. Hence, we can easily see that $COST_{\textbf{p'}}(A_{\textbf{p'},1},A_{\textbf{p'},2}) \ge COST_{\textbf{p}}(A_{\textbf{p},1},A_{\textbf{p},2})$.\par

In conclusion, $\frac{COST_{\textbf{p'}}(A_{\textbf{p'},1},A_{\textbf{p'},2})}{COST_{\textbf{p'}}(opt_{\textbf{p'},1},opt_{\textbf{p'},2})} \ge \frac{COST_{\textbf{p}}(A_{\textbf{p},1},A_{\textbf{p},2})}{COST_{\textbf{p}}(opt_{\textbf{p},1},opt_{\textbf{p},2})}$. Hence, the claim is right. $\hfill\blacksquare$ 

\par\vspace{1ex}\noindent\textbf{\Large Observation 2.3}\vspace{1ex}\par
We claim: for any preference profile \textbf{p}, $COST_{\textbf{q}}(s_l, s_r) \le COST_{\textbf{p}}(opt_{\textbf{p},1},opt_{\textbf{p},2})$.\par

Proof: $COST_{\textbf{q}}(s_l, s_r) \le COST_{\textbf{q}}(opt_{\textbf{p},1},opt_{\textbf{p},2}) \le COST_{\textbf{p}}(opt_{\textbf{p},1},opt_{\textbf{p},2})$. $\hfill\blacksquare$\\

Before we analyze the approximation rate of Mechanism 2.1, we do some preparation work.\par
First, by Observation 2.2, we can assume $\forall i, p_i \in \{\{F_1\},\{F_2\}\}$. We divide all agents into $S_1$ and $S_2$, where $S_k=\{i|p_i=\{F_k\}\}, k=1,2$. We can find that $opt_{\textbf{p},k}$ is the median of $\{x_i|i \in S_k\}$.\par

For simplicity, we introduce more denotations:
\begin{itemize}
\item For two point sets $S$ and $T$, we denote $d(S,T) = \sum\limits_{p \in S} \sum\limits_{q \in T} dist(p,q)$.
\item For a point set $S$ and a point $q$, we denote $d(S,q) = \sum\limits_{p \in S} dist(p,q)$. 
\item We denote $s_{mid}$ as the mid point of $s_l$ and $s_r$. Without loss of generality, we can assume $s_l \le s_r$.
\item As shown in the following statements, \textbf{p} is fixed. Hence, we leave out \textbf{p} in the denotations and let:
	\begin{itemize}
		\item $OPT_i = d(S_i, opt_i)$, $i = 1,2$. $OPT = OPT_1 + OPT_2$. i.e. $OPT = COST_{\textbf{p}}(opt_1,opt_2)$.
		\item $BEST_i = \sum\limits_{p \in S_i} \min \{dist(p, s_l), dist(p, s_r)\}$, $i = 1,2$. $BEST = BEST_1 + BEST_2$. i.e. $BEST = COST_{\textbf{q}}(s_l,s_r)$.
		\item $COST_i = min\{d(S_i, s_l), d(S_i, s_r)\}$, $i = 1,2$. $COST = COST_1 + COST_2$. i.e. $COST = COST_{\textbf{p}}(A_1,A_2)$.
		\item $\Delta_i = \frac{1}{2} (COST_i - OPT_i)$, $i = 1,2$. $\Delta = \Delta_1 + \Delta_2$.
	\end{itemize}
\end{itemize}

\par\vspace{1ex}\noindent\textbf{\Large Theorem 3}\vspace{1ex}\par
Theorem: Mechanism 2.1 is 3-approximated.\par
Proof: We focus on $COST - OPT$.\par
Consider the case that $opt_1$ lies on the left of $s_{mid}$. By definition, $COST_1 - OPT_1 \le d(S_1, s_l) - d(S_1, opt_1)$. \par
We assume $|S_1|$ is even. (Otherwise, we duplicate all agents and approximation rate will not change.) It is easy to see that half of points in $S_1$ lies on the left side of $opt_1$ and half of points in $S_1$ lies on the right side of $opt_1$. We match them into pairs $(u_i,v_i)$, $u_i$ is on the left of $opt_1$, $v_i$ is on the right of $opt_1$.\par

\begin{figure}[htbp]
\centering
\includegraphics[height=5cm]{fig1.png}
\label{figure1}
\end{figure}

We assume $opt_1$ lies on the right of $s_l$ and find an interesting thing: $d(\{u_i,v_i\},s_l)-d(\{u_i,v_i\},opt_1)$ equals to 0 when $u_i$ is on the left of $s_l$ and equals to 2$dist(u_i,s_l)$ when $u_i$ is on the right of $s_l$. Noticing the assumption that $opt_1$ lies on the left of $s_{mid}$, we have:
\begin{align*}
		&COST_1 - OPT_1 \\
		\le &d(S_1, s_l) - d(S_1, opt_1)\\
		= &\sum\limits_{i \in S_1 \ \land \ x_i \in [s_l,opt_1]} 2 \cdot dist(x_i, s_l)\\
		\le &2 \cdot BEST_1
\end{align*}

The case $opt_1$ lies on the left of $s_l$ and the case $opt_1$ lies on the right of $s_{mid}$ are similar.\par
We use the same analyzation and we will have: 
\begin{equation*}
	COST_2 - OPT_2 \le 2 \cdot BEST_2.
\end{equation*}\par
Together, we have $COST - OPT \le 2 \cdot BEST \le 2 \cdot OPT$, which implies $COST\le 3 \cdot OPT$. $\hfill\blacksquare$\\

\par\vspace{1ex}\noindent\textbf{\Large Observation 4}\vspace{1ex}\par
We provide a lower bound for the approximation ratio of Mechanism 2.1.\par
We assume there are $N$ agents locating at $x=0$ with preference $\{F_1\}$, $k \cdot N$ agents locating at $x=1$ with preference $\{F_1\}$ and $\infty$ agents locating at $x=1+y$ with preference $\{F_2\}$. If we let $y < \frac{1}{k}$, we will find $s_l = 0$ and $s_r=1+y$. It is easy to find that the optimal cost is $N$ when $k>1$, while the cost the mechanism 2.1 provides is $\min(kN, kN \cdot y + N \cdot (1+y))$. The approximation ratio will be maximum when $y$ is almost $\frac{1}{k}$ and $k=1+1+\frac{1}{k}$. It is easy to find that when $k=1+\sqrt{2}$, we will have a instance with an approximation ratio = $1+\sqrt{2}$.

\par\vspace{1ex}\noindent\textbf{\Large Analyzation 5}\vspace{1ex}\par
To gain a better upperbound, we should analyze carefully.\par
We still focus on $\Delta_1$. Without loss of generality, we assume $opt_1$ is on the left of $s_{mid}$. we denote $s_c$ as the point between $s_l$ and $s_{mid}$ that lets $dist(s_c,s_{mid}) = c \cdot dist(s_l,s_c)$, where $c$ is a constant parameter. Then we divide the problem into 3 cases:
\begin{enumerate}
	\item $opt_1$ lies on the left of $s_l$.
	\item $opt_1$ lies between $s_c$ and $s_{mid}$.
	\item $opt_1$ lies between $s_l$ and $s_c$.
\end{enumerate}\par
We just analyze these 3 cases one by one.\par

\textbf{Case 1:}\par
\begin{figure}[htbp]
\centering
\includegraphics[height=5cm]{case1.png}
\label{figure1}
\end{figure}\par

In this case, we divide the agents $S_1$ into four point sets: $X_1$, $X_2$, $X_3$ and $X_4$.\par
\begin{enumerate}
	\item $X_1$ contains the point on the left of $opt_1$.
	\item $X_2$ contains the point between $opt_1$ and $s_l$.
	\item $X_3$ contains the point between $s_l$ and $s_{mid}$.
	\item $X_4$ contains the point on the right of $s_{mid}$.
\end{enumerate}\par
By the definition of $\Delta_1$ and the analyzation in Thereom 3, we have:
\begin{equation*}
	\Delta_1 = d(X_2, s_l) \le d(X_1, s_l). \quad (|X_1| = |X_2| + |X_3| + |X_4|).
\end{equation*}\par
We notice that, in this case, we have:
\begin{align*}
	BEST_1 &= d(X_1, s_l) + d(X_2, s_l) + d(X_3, s_l) + d(X_4, s_r) \\
		   &\ge d(X_1, s_l) + d(X_2, s_l) \\
		   &\ge 2 \cdot d(X_2, s_l) \\
		   &= 2 \cdot \Delta_1.
\end{align*}\par
This means that we have $\Delta_1 \le \frac{1}{2} BEST_1$.

\textbf{Case 2:}\par
\begin{figure}[htbp]
\centering
\includegraphics[height=5cm]{case2.png}
\label{figure1}
\end{figure}\par

In this case, we divide the agents $S_1$ into five point sets: $X_1$, $X_2$, $X_3$, $X_4$ and $X_5$.\par
\begin{enumerate}
	\item $X_1$ contains the point between $s_l$ and $opt_1$.
	\item $X_2$ contains the point between $s_{mid}$ and $s_r$.
	\item $X_3$ contains the point between $opt_1$ and $s_{mid}$.
	\item $X_4$ contains the point on the left of $s_l$.
	\item $X_5$ contains the point on the right of $s_r$.
\end{enumerate}\par
By the definition of $\Delta_1$ and the analyzation in Thereom 3, we have:
\begin{equation*}
	\Delta_1 = \min \{d(X_1,s_l), d(X_3, s_r) + d(X_2, s_r)\}
\end{equation*}\par

In this case,
\begin{align*}
	BEST_1 &= d(X_1,s_l) + d(X_2, s_r) + d(X_3, s_l) + d(X_4, s_l) + d(X_5, s_r)\\
		   &\ge d(X_1,s_l) + d(X_2, s_r) + d(X_3, s_l).
\end{align*}\par

By the definition of $s_{mid}$, $s_c$ and the assumption in this case that $opt_1$ lies on the right of $s_c$, we have: 
\begin{align*}
	d(X_3, s_r) + d(X_2, s_r) &= d(X_3, s_l) + 2 \cdot d(X_3,s_{mid}) + d(X_2, s_r)\\
							 &\le d(X_3, s_l) + 2c \cdot d(X_3, s_l) + d(X_2, s_r)\\
							 &= (2c+1) \cdot d(X_3, s_l) + d(X_2, s_r)\\
							 &\le (2c+1) \cdot (d(X_3, s_l) + d(X_2, s_r)).
\end{align*}\par
Now, if $d(X_1,s_l) \le \frac{2c+1}{2c+2} BEST_1$, we have:
\begin{equation*}
	\Delta_1 \le d(X_1,s_l) \le \frac{2c+1}{2c+2} BEST_1.\\
\end{equation*}\par
Otherwise, $d(X_1,s_l) > \frac{2c+1}{2c+2} BEST_1$. Hence, we have: 
\begin{align*}
	\Delta_1 &\le d(X_3, s_r) + d(X_2, s_r)\\
			 &\le (2c+1) \cdot (d(X_3, s_l) + d(X_2, s_r))\\
			 &\le (2c+1) \cdot (BEST_1 - d(X_1,s_l))\\
			 &< (2c+1) \cdot \frac{1}{2c+2} BEST_1.
\end{align*}\par
Together, we have $\Delta_1 \le \frac{2c+1}{2c+2} BEST_1$.

\textbf{Case 3:}\par
\begin{figure}[htbp]
\centering
\includegraphics[height=5cm]{case3.png}
\label{figure1}
\end{figure}\par

In this case, we divide the agents $S_1$ into the same five point sets defined in \textbf{Case 2}.\par
In this case, like Case 2, we have:
\begin{align*}
	&\Delta_1 = \min \{d(X_1,s_l), d(X_3, s_r) + d(X_2, s_r)\}, \\
	&BEST_1 = d(X_1,s_l) + d(X_2, s_r) + d(X_3, s_l) + d(X_4, s_l) + d(X_5, s_r).
\end{align*}\par
We let $\alpha$ be a constant parameter.\par
Now, if $d(X_2, s_r) + d(X_3, s_l) \ge \alpha \cdot d(X_1,s_l)$, we have:
\begin{align*}
	BEST_1 &\ge d(X_1,s_l) + d(X_2, s_r) + d(X_3, s_l)\\
		   &\ge (1+ \alpha) \cdot d(X_1, s_l)\\
		   &\ge (1+ \alpha) \cdot \Delta_1
\end{align*}\par
i.e. $\Delta_1 \le \frac{1}{1+\alpha} BEST_1$.\par
Otherwise, we have:
\begin{align*}
	\alpha \cdot d(X_1, s_l) &> d(X_2, s_r) + d(X_3, s_l)\\
		   					 &\ge d(X_2, s_r) + |X_3| \cdot dist(opt_1, s_l)\\
		 				     &\ge d(X_2, s_r) + \frac{|X_3|}{|X_1|} \cdot d(X_1, s_l).
\end{align*}\par
Now, we focus on the lower bound of $OPT_1$:
\begin{align*}
	OPT_1 &= d(S_1, opt_1)\\
		  &\ge d(X_2 \cup X_5, opt_1)\\
		  &= |X_2| \cdot dist(opt_1, s_r) - d(X_2, s_r) + d(X_5, opt_1)\\
		  &\ge (|X_2|+|X_5|) \cdot dist(opt_1, s_r) - d(X_2, s_r)\\
		  &\ge (|X_1|-|X_3|) \cdot dist(opt_1, s_r) - d(X_2, s_r)\\
		  &\ge (|X_1|-|X_3|) \cdot \frac{2c+1}{2c+2} \cdot dist(s_l, s_r) - d(X_2, s_r) \quad \quad (d(X_1, s_l) \le |X_1| \cdot \frac{dist(s_l,s_r)}{2c+2})\\
		  &\ge (2c+1) \cdot \frac{|X_1|-|X_3|}{|X_1|} \cdot d(X_1, s_l) - d(X_2, s_r)\\
		  &= (2c+1) \cdot d(X_1, s_l) - ((2c+1) \cdot \frac{|X_3|}{|X_1|} \cdot d(X_1, s_l)+ d(X_2, s_r))\\
		  &\ge (2c+1) \cdot d(X_1, s_l) - (2c+1)(\frac{|X_3|}{|X_1|} \cdot d(X_1, s_l)+ d(X_2, s_r))\\
		  &\ge (2c+1) \cdot d(X_1, s_l) - (2c+1) \cdot \alpha \cdot d(X_1, s_l)\\
		  &= (2c+1) \cdot (1 - \alpha) \cdot d(X_1, s_l)\\
		  &\ge (2c+1) \cdot (1 - \alpha) \cdot \Delta_1.
\end{align*}\par
Hence, we have $\Delta_1 \le \frac{1}{(2c+1) \cdot (1-\alpha)} OPT_1$.\par
Now, we consider the tradeoff.\par
We let $c=1$ and $\alpha = \frac{1}{2c+1}$. Therefore, for $\Delta_1$, we have one of the following:
\begin{enumerate}
	\item $\Delta_1 \le \max \{\frac{1}{2}, \frac{2c+1}{2c+2}, \frac{1}{1 + \alpha}\} \cdot BEST_1 = \frac{3}{4}BEST_1$.
	\item $\Delta_1 \le \frac{1}{(2c+1) \cdot (1-\alpha)} OPT_1 = \frac{1}{2} OPT_1$.
\end{enumerate}\par
It is easy to see that we have the same bound for $\Delta_2$.\par
Without loss of generality, we assume $BEST_1 \ge BEST_2$. We divide the discussion into 4 cases:\par
\textbf{Case 1:} $\Delta_1 \le \frac{3}{4}BEST_1$, $\Delta_2 \le \frac{3}{4}BEST_2$\par
We have $\Delta = \Delta_1 + \Delta_2 \le \frac{3}{4} (BEST_1 + BEST_2) = \frac{3}{4} BEST \le \frac{3}{4} OPT$.\par

\textbf{Case 2:} $\Delta_1 \le \frac{1}{2}OPT_1$, $\Delta_2 \le \frac{1}{2}OPT_2$\par
We have $\Delta = \Delta_1 + \Delta_2 \le \frac{1}{2} (OPT_1 + OPT_2) = \frac{1}{2}OPT$.\par

\textbf{Case 3:} $\Delta_1 \le \frac{1}{2}OPT_1$, $\Delta_2 \le \frac{3}{4}BEST_2$\par
We have:
\begin{align*}
\Delta &= \Delta_1 + \Delta_2\\
	   &\le \frac{1}{2} OPT_1 + \frac{3}{4}BEST_2\\
	   &\le \frac{1}{2} OPT + \frac{3}{8}(BEST_1 + BEST_2)\\
	   &= \frac{1}{2} OPT + \frac{3}{8}BEST\\
	   &\le \frac{1}{2} OPT + \frac{3}{8}OPT\\
	   &= \frac{7}{8}OPT.
\end{align*}\par

\textbf{Case 4:} $\Delta_1 \le \frac{3}{4}BEST_1$, $\Delta_2 \le \frac{1}{2}OPT_2$\par
\begin{align*}
\Delta &= \Delta_1 + \Delta_2\\
	   &\le \frac{3}{4} BEST_1 + BEST_2\\
	   &= \frac{3}{4} BEST_1 + \frac{1}{8}BEST_2 + \frac{7}{8}BEST_2\\
	   &\le \frac{3}{4} BEST_1 + \frac{1}{8}BEST_1 + \frac{7}{8}BEST_2\\
	   &= \frac{7}{8} (BEST_1 + BEST_2)\\
	   &= \frac{7}{8} BEST.\\
	   &\le \frac{7}{8} OPT.
\end{align*}\par
Together, we have $\Delta \le \frac{7}{8} OPT$.\par
Therefore, we have $COST -OPT = 2 \cdot \Delta \le 2 \cdot \frac{7}{8} OPT = \frac{7}{4} OPT$. i.e. $COST \le 2.75 \cdot OPT$. $\hfill\blacksquare$\\
